Filament Eruption Driving EUV Loop Contraction then Expansion above a Stable Filament

We analyze the observations of EUV loop evolution associated with the filament eruption located at the border of an active region. The event SOL2013-03-16T14:00 was observed with a large difference of view point by the Solar Dynamics Observatory and Solar Terrestrial Relations Observatory --A spacecraft. The filament height is fitted with the sum of a linear and exponential function. These two phases point to different physical mechanisms such as: tether-cutting reconnection and a magnetic instability. While no X-ray emission is reported, this event presents the classical eruption features like: separation of double ribbons and the growth of flare loops. We report the migration of the southern foot of the erupting filament flux rope due to the interchange reconnection with encountered magnetic loops of a neighbouring AR. Parallel to the erupting filament, a stable filament remains in the core of active region. The specificity of this eruption is that coronal loops, located above the nearly joining ends of the two filaments, first contract in phase, then expand and reach a new stable configuration close to the one present at the eruption onset. Both contraction and expansion phases last around 20 min. The main difference with previous cases is that the PIL bent about 180 deg around the end of the erupting filament because the magnetic configuration is at least tri-polar. These observations are challenging for models which interpreted previous cases of loop contraction within a bipolar configuration. New simulations are required to broaden the complexity of the configurations studied.

==> MS_labels.tex <==


\sect{Introduction}
\sect{Observations}
   \sect{Overview}
   \sect{Magnetic}
   \sect{Filament}
   \sect{Kinematics}
     \eq{h(t)}
     \eq{t_start}
   \sect{Loop}
\sect{Physical}
   \sect{Physical_Magnetic}
   \sect{Physical_Loop}
\sect{Conclusion}

 1 \fig{evolution}
 2 \fig{MGN171}
 3 \fig{mag}
 4 \fig{ht}
 5 \fig{stereo}
 6 \fig{loops}
 7 \fig{slice_171}
 8 \fig{slice_193}
 

 %%% labels
 Fil$_1$  Fil$_2$
 L$_1$  L$_2$  L$_3$
 
Evolution:
 present at https://www.youtube.com/watch?v=8ltspe3w714
 tStartErupt    13:30 UT: onset filament eruption (304)   
 tVt=c          13:37 UT: V_linear = V_exp
 tStartContrac  13:40 UT: onset loop contraction (171,193), duration: 22 min 
                14:02 UT: onset loop expansion (171,193), duration: 15/25 min  
 
                13:59 UT: onset ribbons below filament (171 movie)
 
 Slice S2
        14:18 UT: flare ribbons start to be bright and separate  (171,193)
        14:34 UT: flare loop start
  
% Commands for figures, sections & equations,
\newcommand{\fig}[1]{Figure~\ref{fig_#1}}
\newcommand{\figS}[1]{Figures~\ref{fig_#1}}
\newcommand{\figs}[2]{Figures~\ref{fig_#1} and \ref{fig_#2}}
\newcommand{\figss}[2]{Figures~\ref{fig_#1}-\ref{fig_#2}}
\newcommand{\sect}[1]{Section~\ref{sect_#1}}
\newcommand{\sects}[2]{Sections~\ref{sect_#1} and~\ref{sect_#2}}
\newcommand{\eq}[1]{Equation~(\ref{eq_#1})}
\newcommand{\eqs}[2]{Equations~(\ref{eq_#1}) and (\ref{eq_#2})}
\newcommand{\eqss}[2]{Equations~(\ref{eq_#1}) - (\ref{eq_#2})}
\newcommand{\eqsss}[3]{Equations~(\ref{eq_#1}), (\ref{eq_#2}) and (\ref{eq_#3})}
\newcommand{\tab}[1]{Table~\ref{tab_#1}}
\newcommand{\BE}{\begin{equation}}
\newcommand{\EE}{\end{equation}}
\newcommand{\BA}{\begin{eqnarray}}
\newcommand{\EA}{\end{eqnarray}}

% General definitions for derivatives
\newcommand{\f}[2]{{\ensuremath{\mathchoice%
        {\dfrac{#1}{#2}}
        {\dfrac{#1}{#2}}
        {\frac{#1}{#2}}
        {\frac{#1}{#2}}
        }}}
\newcommand{\Int}[2]{\ensuremath{\mathchoice%
        {\displaystyle\int_{#1}^{#2}}
        {\displaystyle\int_{#1}^{#2}}
        {\int_{#1}^{#2}}
        {\int_{#1}^{#2}}
        }}
\newcommand{\curl}{ {\bf \nabla } \times}
\newcommand{\rmd}{{\rm d }}
\renewcommand{\div}[1]{ {\bf \nabla}. #1 }
\newcommand{\grad}{  {\bf \nabla} }
%\newcommand{\pardiff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pder}[2]{\f{\partial #1}{\partial #2}}
\newcommand{\der}[2]{\f{\rmd \, #1}{\rmd \, #2}}

% General definitions of symbols 
\newcommand{\arcsec}{''} 
\newcommand{\degree}{^\circ} 
\newcommand{\kms}{km s$^{-1}$} %{km/s} 
\newcommand{\Rsun}{$R_{\odot}$}  
\newcommand{\uvec}[1]{\hat{\bf #1}}
%\renewcommand{\vec}[1]{ \textit{\textbf{#1}} }

% text
\newcommand{\cf}{\textit{cf.}}
\newcommand{\eg}{\textit{e.g.,}}
\newcommand{\etal}{\textit{et al.}}
\newcommand{\ie}{\textit{i.e.,}}
\newcommand{\insitu}{\textit{in situ}}
\newcommand{\vs}{\textit{vs}}
\newcommand{\vv}{\textit{v.v.}}
\newcommand{\de}{$\Delta$} 
\newcommand{\ha}{H$\alpha$}


